Sketchy With a Chance of Adoption: Can Sketch-Based Telemetry Be Ready for Prime Time?

Sketching algorithms or sketches have emerged as a promising alternative to the traditional packet sampling-based network telemetry solutions. At a high level, they are attractive because of their high resource efficiency and accuracy guarantees. While there have been significant recent advances in various aspects of sketching for networking tasks, many fundamental challenges remain unsolved that are likely stumbling blocks for adoption. Our contribution in this paper is in identifying and formulating these research challenges across the ecosystem encompassing network operators, platform vendors/developers, and algorithm designers. We hope that these serve as a necessary fillip for the community to enable the broader adoption of sketch-based telemetry.

==> sections/controlplane.tex <==
\section{Control Plane}









\subsection{Limitations of Existing Work}
Existing efforts on sketch-based telemetry, such as UnivMon~\cite{univmon},  SketchVisor~\cite{SketchVisor}, Elastic Sketch~\cite{elasticsketch}, have tackled on the network-wide resource allocation problem that distributes sketch capabilities among a network to offer ``one-big-switch'' telemetry abstraction using minimized resource footprints. However, these efforts fall short in one or more of the following dimensions: (1) {\em Traffic-awareness} to optimize the global memory usage and packet processing performance based on traffic demands and expect traffic characteristics; (2) {\em Device heterogeneity} to optimize the global memory usage and packet processing performance based on diverse device capabilities. As a result, existing network-wide solutions utilize excessive compute and memory resources compared to the optimal possible resource allocation.  For instance, \alan{TODO: pending an quantitative example from Anup.}


\subsection{Open Problems}
\begin{insight}[Optimized Sketch Configuration]
Given workload characteristics $\mathcal{T_r}$ and a sketch $s$ with accuracy requirements, can we output a minimal platform-agnostic memory configuration for $s$ that meets the accuracy requirement?
\end{insight}

Problem 3 is about determining a minimal memory configuration meeting certain accuracy requirement for a sketch and a given type of workload characteristics (e.g., skewness, number of flows). Traditionally, the theoretical analysis of a sketch can help determine a memory configuration to fulfill the accuracy requirement in the worst-case. However in practice, this memory-accuracy tradeoff shown in the analysis is ``loose'': If we only need to support workloads with predictable characteristics (which are usually better than the worst case), we should be able to search for a configuration that both consumes smaller memory space and meets the accuracy requirement. By solving the 


\begin{insight}[Resource Optimization]
Given a set of sketches $\mathcal{S}$ with dynamically changing accuracy requirements $\mathcal{O_A}$ and performance requirements $\mathcal{O_P}$,
traffic characteristics $\mathcal{T_r}$, topology information $\mathcal{T}$, and devices instances $\mathcal{D}$, can we output the resource configuration $r_{s,d}$ for all $s,d$ within a time budget such that $\sum_s\sum_d r_{s,d}$ is minimized and $\forall s \in {S}$ meets $\mathcal{O_A}$ and $\mathcal{O_P}$?
\end{insight}
Problem 4 is about minimizing the network-wide sketch resource usage across a network of heterogeneous devices. Given the requirements of accuracy and packet processing performance, the goal of this optimization is to decide which sketch should be placed on which device and how much resource should be allocated for each sketch on the device, such that the total resource usage is minimized. 
In this problem, the traffic characteristics, path information (topology), and device specifications will play a role in the sketch place and resource allocation. For example, if an OD-path has known traffic characteristics and different types of devices to place the telemetry capabilities, placing the same sketch into different hardware (e.g., switch and server CPU) will has different memory and compute resource usages.

\begin{insight}[Maximum Performance]
Given a set of sketches $\mathcal{S}$ with requirements $\mathcal{O_A}$, topology information $\mathcal{T}$, and devices $\mathcal{D}$, can we output resource configuration $r_{s,d}$ for all $s,d$ such that $\sum_s\sum_d l_{s,d}$ is minimized and $\forall s \in \mathcal{S}$ meets $\mathcal{O_A}$?
\end{insight}
Problem 5 is to provide an optimized network-wide sketch placement and resource allocation that meet the device resource constraints and minimizes the packet processing overhead. In this optimization, we aim at deploying a telemetry solution to handle largest possible volume of traffic for given queries, which potentially offers us the ability to monitor bursty traffic.



==> sections/dataplane.tex <==
\section{Data Plane Implementation}

\subsection{Limitations of Existing Work}
\alan{TODO: A concrete measurement on the inefficient sketch implementation on P4. }

\subsection{Open Problems}
\begin{insight}[Sketch Implementation] 
Given $r_{s,d}$ for (potentially new) sketch instance $s$ and device instance $d$, can we generate sketch implementation $c_{s,d}$ such that actual resource usages $m_{s,d}$ and $l_{s,d}$ are minimized  ?
\end{insight}

Problem 6 is about building a tool to automatically generate sketch hardware implementation for any sketch resource configuration and device instance. At the moment, it requires tremendous joint efforts from platform and algorithms developers to deliver an resource- and performance-optimized sketch implementation per hardware target. Sometimes, achieving even a feasible implementation is difficult~\cite{SketchVisor,univmon}. Thus, we envision this tool (e.g., a specialized code compiler) to take as input algorithm definition and configuration defined in a high-level language (e.g., P4), and automatically output an implementation that is optimized for a particular hardware target. With such a tool, algorithm developers will not need to worry about how to implement a current or future sketching algorithm into a hardware architecture and platform developers will not worry about understanding the algorithmic details in order to implement the sketches.
\antonis{unclear to me from this text why P4 is lacking here. After reading this para, it felt like you were describing P4 again}

\begin{insight}[Implementation Optimization]
Given $r_{s,d}$ for all sketch configuration $s \in \mathcal{S}$ and device instance $d \in \mathcal{D}$, can we generate sketch implementation $c_d$ for device $d$ such that the device actual resource usage $\sum_s m_{s,d}$ and $\sum_s l_{s,d}$ are minimized?
\end{insight}

Problem 7 can be considered as a generalized version of Problem 6. This problem is about optimizing the sketch implementation on a device when multiple sketch instances are present. Our observation is that many sketches share common primitive operations (hash computation, counter updates, etc.), and we expect that the actual memory usage and packet processing performance on a device $d^*$ can be further optimized to less than $\sum_s r_{s,d^*}$.




==> sections/frontend.tex <==
\section{Unified Front End}

\begin{table}[t]
\centering
\footnotesize

\begin{tabular}{ cl }
\toprule
\textbf{Constants} & Definition\\
\midrule
$\mathcal{Q}$ & Set of telemetry queries\\
$\mathcal{O_A}$ & Set of accuracy requirements, \\
& ~~e.g., accuracy target and confidence level\\
$\mathcal{O_P}$ & Set of performance requirements,\\
& ~~e.g., packet rate performance\\
$\mathcal{T}$ & Topology information, e.g., links and devices\\
$\mathcal{D}$ & Set of device instances with resource constraints, \\
& ~~e.g., SmartNIC with 4 engines and 10MB SRAM \\
$\mathcal{T_r}$ & Workload characteristics, e.g., distribution \\

\end{tabular}
\begin{tabular}{ cl }
\toprule
\textbf{Variables} & Definition\\
\midrule
${S}$ & Set of sketch instances with memory configurations \\ 
$r_{s,d}$ & Resource config. for sketch s on device $d$ instance \\
$l_{s,d}$ & Processing latency for sketch s on device $d$ instance\\
$c_{s,d}$ & Implementation of sketch $s$ on device $d$\\
$c_{d}$ & Implementation of all sketches on device $d$\\
$m_{s,d}$ & Actual memory usage of device $d$ from $c_{d}$ \\
\\

\bottomrule
\end{tabular}
\caption{Summary of parameters and variables in open problems.}
\label{tab:definition}
\end{table}









\subsection{Limitations of Existing Work}

\vyas{perhaps don't harp on this too much or call out explicit attention to the limitations of the existing work. in some sense we are already setting up that expectation in sec 1. just dive into the detailed problems and then highlight why/where existing stuff falls short?}

\antonis{I would drop the subsection header - limitations of prior work-. I agree with Vyas' comment and also I personally don't like to see a subsection right under a section header (but that's just my pet-peeve. I think the same text would be perfectly suitable as intro to the section}

\prs{I agree: focus on open problems and discussion limitations of previous work in that context.}

\hun{I have another question - 3. overview section and all of problems in section 4 - 6 sounds great. The thing is that some of problems themselves suggest a solution of "automation" (e.g., problem6/7 suggest process automation to replace the role of platform developer). I think it would be good to setup this clearly in advance by saying either we are suggesting only problems or we talk about problems with solutions by the framework even though it is a high level. Or in other words, do we envision that the problems are solved in manual effort by collaborative work between algo developer and platform developer? or we envision that all of the problems are solved by automated manner by the framework so that communication is not needed anymore.}


Traditionally, sketch-based telemetry systems are designed under a ``narrow-scope'' 
assumption with respect to the generality of queries they can support. Specifically, 
existing frameworks are either designed to support only one type of queries~\cite{sigmod_paper}
or assume that the operator will determine at query time the appropriate (available) 
sketch for each query. For example, to detect super-spreaders  (i.e., SrcIPs that connect
to many distinct DstIPs), the user needs to make a choice between X,Y sketches whereas
to detect heavy hitters they need to choose between A,B sketches~\cite{apache_druid}. 
As a result, developing a unified user-front end for such telemetry systems was, to the
best of our knowledge, never seen as a key design priority.   


The closest efforts to our goal are OpenSketch~\cite{OpenSketch} and Sonata~\cite{sonata}.
OpenSketch~\cite{OpenSketch} is sketch-based telemetry library in NetFPGA, including
Count-Min~\cite{CMSketch}, K-ary sketch~\cite{k-ary}, and reversible sketch~\cite{ReversibleSketch}.
Although OpenSketch showed a way to program its controller in order to add a new measurement
program, it remains unclear if OpenSketch will be able to define all existing or future 
sketch-based measurement queries. While Sonata provides a unified interface to query telemetry
statistics, their interface is based on a SQL-alike language to specify the detailed user-level queries. However, Sonata does not consider sketches as their monitoring primitives and overly complicate the query definitions for sketches. Similarly, other efforts such as NetQRE~\cite{netqre} and Marple~\cite{marple} provide query interfaces for network operators to specify their telemetry policies and a different set of telemetry metrics (e.g., network performance) but they were designed without considering sketch abstractions as telemetry primitives and we are unsure if they can support sketch-based queries or are overly complicated to define a sketch-based telemetry query.




\subsection{Open Problems}

\begin{insight}[Query Language]
Can we design a high-level declarative language that can precisely define telemetry queries
$\mathcal{Q}$ supported by sketches?
\end{insight}

Problem 1 is about designing a declarative query language specifically for sketch-based telemetry 
systems. With
the growth of sketch functionality, it becomes much more difficult than ever for network operators to study the details of sketching algorithms in the telemetry system in order to properly define the query input and output. To let network operators use sketch-based telemetry systems easily, we ideally need a high-level querying language that is expressive enough to cover the broadest possible set of queries while hiding the intricacies of the execution from the user. Specifically, the user 
should be able to conceptually describe the characteristics of the telemetry query they want 
to execute (e.g., type of estimation, aggregation of data necessary, required accuracy constraints) without having to explicitly specify the mechanism of execution. 





\begin{insight}[Traffic-Oblivious Compilation] For all workload characteristics $\mathcal{T_r}$,  instances $D$, and a set of queries $\mathcal{Q}$, can we build a compiler that translates $\mathcal{Q}$ into a set of platform-agnostic sketch configurations ${S}$ that meet requirements $\mathcal{O_A}$? 
\end{insight}

\antonis{I have a concern here: I got slightly confused here after reading your definition of problem 2 and problem 3. I think you need to bring the discussion of "different workload params produce different accuracy guarantees" here and elevate more the point that at this step you produce a set of candidate sketches. There's significant overlap right now between 2-3 and it's unclear from the current text where you draw the line. }

Problem 2 is about translating telemetry queries into a composition of sketch configurations that can meet the accuracy requirements from the queries, regardless of traffic workload characteristics and hardware platforms. This is possible because the accuracy guarantee of sketches is hardware agnostic and only depends on the memory configuration. Thus, we can potentially leverage the theoretical analysis to provide sketch memory configuration treating the network-wide devices as a ``one-big-switch'' such that the worst-case accuracy requirements on this switch can be guaranteed.  For example, if a query specifies a heavy hitter task with $98\%$ accuracy and 0.99 confidence level, we expect a compiler to generate a minimized sketch configuration (e.g., Count-Min Sketch with $r\times d$ counters) that maintains errors $\le 2\%$ with 0.99 probability under any workload distribution and hardware platform.    

This problem can be considered as a first compilation step towards a network-wide device-aware resource allocation in the control plane which usually requires target-agnostic memory configurations and corresponding performance characteristics on each hardware target as input.


==> sections/overview.tex <==
\section{Overview}
\vyas{not sure id call this motivation/overview. we can shrink this and directly jump into the open problems etc. just do setup notation/and the stakeholder definition here. these are not "scenarios" as such }

\prs{Maybe move the subsection on motivating scenarios to the previous section and kill the rest?  Motivating scenarios should be high level.}

\hun{We use (platform)/(network devices) as the same meaning, but the usage can be subtle that might confuse readers.}

In this section, we first highlight several scenarios from the stakeholders involving in the research of sketch-based network telemetry, such as network operator, algorithm developer, and platform developer, and then discuss a sketch-based telemetry framework that designed to meet the requirements from parties.

\subsection{Stakeholders and  Requirements} 

\paraf{Network operator.} Network operators rely on real-time telemetry information to make timely control decisions in order to improve network reliability, performance, and security. When managing the network, the operator may want to obtain network-wide information from one or a set of telemetry tasks, such as global heavy hitter flows, distinct flows, and entropy changes. However, network operators may not have the knowledge about the sketch design and implementation. Then they cannot decide which sketches should be used for the required telemetry tasks and how to configure the sketches to meet certain accuracy goals. 

Ideally, network operators should be only required to provide high-level queries and telemetry objectives without knowing the underlying details about sketches. For example, the operator may specify queries as the following. The telemetry system should be able to identify whether the queries can be fully supported by the existing library of sketches. If better or new sketches are needed, the telemetry system should pass these information to algorithm developers.
\begin{figure}[h]
\centering
    \begin{minipage}[t]{.49\textwidth}
\textbf{Q1: Return 5-tuple 0.005-heavy hitters from all flows}
\begin{codefragment2}
FlowKey = (SrcIP,SrcPort,DstIP,DstPort,Proto)
C="Select HeavyHitter(p.FlowKey,0.05) From *"
return C
  \end{codefragment2}
  \end{minipage}
  \begin{minipage}[t]{.49\textwidth}
  \textbf{Q2: Return distinct DstIP count that a host connects to}
  \begin{codefragment2}
C="Select Distinct(p.dstIP) From *
Where p.srcIP=1.2.3.4"
return C
  \end{codefragment2}
  \end{minipage} 
\label{fig:query_example}
\end{figure}


\para{Algorithm developer.}  Algorithm developers and theorists are the ones who design sketching algorithms to estimate different telemetry metrics. From their perspective, they would like to understand the requirements from network operators and design improved or new sketching algorithms for needed metrics. In practice, it requires tremendous efforts from algorithm developers to obtain the real-world telemetry requirements from network operators and to have their algorithms evaluated in real-world hardware targets with optimized implementations.

Ideally, algorithm developers should have a straightforward way to obtain the telemetry requirements from network operators as their motivation to develop new and improved sketching algorithms. \hun{This points out the difficulty or a communication problem between network operator and algorithm developer. Is it enough to point out current existing problem? or do we have a high level solution for this? If we will suggest automated process in later sections, then above sentence should be like: we should automate those process to remove the need for the communication between algo/network operator developer(?)} Once new algorithms have been designed, we cannot expect algorithm developers to understand network hardware architectures and implement the algorithms by themselves. We should transfer these algorithm definitions to platform developers in order to get them properly implemented in a variety of platforms.  


\para{Platform developer.} There has been a tremendous interest in developing new network devices and platforms with diverse flexibility and packet processing capability. For instance, we have programmable switches, SmartNIC, FPGA, and software switches established in today's network. If platform developers such as network hardware and software developers plan to have sketch primitives deployed on their devices, they want to achieve best possible resource efficiency and guaranteed performance. However, today's sketch design and implementation are far from being optimized~\cite{liu2019nitrosketch} since it is challenging for platform developers to achieve optimally without the help of algorithm developers. 

Ideally, platform developers should implement sketches into every supported hardware platform in an optimized way. We anticipate a mechanism for algorithm and platform developer to jointly contribute their domain-specific knowledge to the sketch implementation without the need for algorithm developer to dig into hardware architecture and the need for platform develop to dig into the algorithmic details. 




\subsection{Sketch-based Telemetry Framework }
Inspired by the different stakeholders in network telemetry, we propose a framework to capture their requirements in participating sketch-based telemetry research. 
As shown in Figure~\ref{fig:overview} \hun{This figure is insightful. One question is that sketch library should be in L1 instead of L2 (Algorithm developer should be linked to L1 accordingly)?}
\para{User front-end:}
\para{Control plane:}
\para{Data plane:}

\begin{figure}[t]
\centering
\includegraphics[width=0.85\linewidth]{figures/overview.pdf}
\caption{Sketch-based Telemetry Framework}
\label{fig:overview}
\end{figure}
